RadEdit: stress-testing biomedical vision models via diffusion image editing

Biomedical imaging datasets are often small and biased, meaning that real-world performance of predictive models can be substantially lower than expected from internal testing. This work proposes using generative image editing to simulate dataset shifts and diagnose failure modes of biomedical vision models; this can be used in advance of deployment to assess readiness, potentially reducing cost and patient harm. Existing editing methods can produce undesirable changes, with spurious correlations learned due to the co-occurrence of disease and treatment interventions, limiting practical applicability. To address this, we train a text-to-image diffusion model on multiple chest X-ray datasets and introduce a new editing method RadEdit that uses multiple masks, if present, to constrain changes and ensure consistency in the edited images. We consider three types of dataset shifts: acquisition shift, manifestation shift, and population shift, and demonstrate that our approach can diagnose failures and quantify model robustness without additional data collection, complementing more qualitative tools for explainable AI.

==> figures/segmentation_bar.tex <==
%         Real data & 0.974\hspace{3.2em} & 6.07\hspace{2.65em} & 0.955\hspace{3.2em} & 11.62\hspace{3.2em} \\
%         Healthy $\overset{\mbox{\tiny edit}}{\rightarrow}$ edema & 0.938 (\textbf{0.036}) & 21.79 (15.72) & 0.919 (\textbf{0.036}) & 22.44 (\textbf{10.82}) \\
%         Healthy $\overset{\mbox{\tiny edit}}{\rightarrow}$ pacemaker & 0.850 (0.124) & 49.81 (43.74) & 0.873 (\textbf{0.082}) & 29.53 (\textbf{17.91})  \\
%         Healthy $\overset{\mbox{\tiny edit}}{\rightarrow}$ consolidation &  0.859 (0.115) & 44.13 (38.06) & 0.881 (\textbf{xyz}) & 29.41 (\textbf{xyz})

\begin{figure}[t]
    \centering
    % \vspace{-1em}
    \begin{subfigure}{0.49\linewidth}
        \resizebox{\linewidth}{!}{
        \begin{tikzpicture}[
          every axis/.style={ % add these settings to all the axis environments in the tikzpicture
            width = 1.38\linewidth,
            height = 5cm,
            ybar stacked,
            ymajorgrids = true,
            major x tick style = transparent,
            ylabel = {},
            yticklabel style={/pgf/number format/fixed},
            xtick = \empty,
            axis line style={draw=none},
            enlarge x limits=0.25,
            bar width=14pt,
            symbolic x coords={
              Edema,
              Pacemaker,
              Consolidation,
            },
          },
        ]

        \draw[myred, line width=1pt] (0,4.37) -- (6.68,4.37);
        \draw[myblue, line width=1pt] (0,3.97) -- (6.68,3.97);

        % Set Hausdorff 0 point. Here as MIMIC-Seg baseline
        \pgfmathsetmacro\hausdorffaxis{0.0}

        % Hausdorff MIMIC-Seg
        % bar shift -10pt here
        \pgfmathsetmacro\mimichausdorffreal{6.07}
        \pgfmathsetmacro\mimichausdorffblank{\mimichausdorffreal-\hausdorffaxis}
        \pgfmathsetmacro\mimichausdorffdema{21.79-\mimichausdorffblank-\hausdorffaxis}
        \pgfmathsetmacro\mimichausdorffpacemaker{49.81-\mimichausdorffblank-\hausdorffaxis}
        \pgfmathsetmacro\mimichausdorffconsolidation{44.13-\mimichausdorffblank-\hausdorffaxis}
        \begin{axis}[
            bar shift=-9pt,
            ymin=0.0, ymax=53.0,
            ylabel={$\Delta$ AHD $\downarrow$},
            at={(0,3.6cm)},
            % ytick={0,20,40},
            yticklabel={
                \pgfmathparse{\tick+\hausdorffaxis}
                \pgfmathprintnumber{\pgfmathresult}
            }
        ]
            \addplot[draw=none] coordinates
            {
                (Edema,\mimichausdorffblank) 
                (Pacemaker,\mimichausdorffblank) 
                (Consolidation,\mimichausdorffblank)
            };
            \addplot[black, fill=myblue] coordinates
            {
                (Edema,\mimichausdorffdema) 
                (Pacemaker,\mimichausdorffpacemaker) 
                (Consolidation,\mimichausdorffconsolidation)
            };
        \end{axis}
        
        % Hausdorff CheXmask
        \pgfmathsetmacro\mimichausdorffreal{11.62}
        \pgfmathsetmacro\mimichausdorffblank{\mimichausdorffreal-\hausdorffaxis}
        \pgfmathsetmacro\mimichausdorffdema{22.44-\mimichausdorffblank-\hausdorffaxis}
        \pgfmathsetmacro\mimichausdorffpacemaker{29.53-\mimichausdorffblank-\hausdorffaxis}
        \pgfmathsetmacro\mimichausdorffconsolidation{29.41-\mimichausdorffblank-\hausdorffaxis}   
        \begin{axis}[
            bar shift=9pt,
             ymin=0.0, ymax=50.0,
            at={(0,3.6cm)},
            hide axis,
        ]
            \addplot[draw=none] coordinates
            {
                (Edema,\mimichausdorffblank) 
                (Pacemaker,\mimichausdorffblank) 
                (Consolidation,\mimichausdorffblank)
            };
            \addplot+[black, fill=myred] coordinates
            {
                (Edema,\mimichausdorffdema) 
                (Pacemaker,\mimichausdorffpacemaker) 
                (Consolidation,\mimichausdorffconsolidation)
            };
            
        \end{axis}

        % \draw[draw=black, line width=0.1em] (0.15,-3.25) rectangle ++(1.93,7.25);
        % \draw[draw=black, line width=0.1em] (2.37,-3.25) rectangle ++(1.93,7.25);
        % \draw[draw=black, line width=0.1em] (4.6,-3.25) rectangle ++(1.93,7.25);

        % \node[] at (1.15,3.3) {\footnotesize Healthy $\overset{\mbox{\tiny edit}}{\rightarrow}$};
        % % \node[] at (1.15,3.0) {$\downarrow$};
        % \node[] at (1.15,2.9) {\footnotesize Oedema};
        % \node[] at (3.35,3.3) {\footnotesize Healthy};
        % \node[] at (3.35,3.0) {$\downarrow$};
        % \node[] at (3.35,2.7) {\footnotesize Pacemaker};
        % \node[] at (5.55,3.3) {\footnotesize Healthy};
        % \node[] at (5.55,3.0) {$\downarrow$};
        % \node[] at (5.55,2.7) {\footnotesize Consolidation};

        \node[] at (1.15,3.3) {\footnotesize Healthy $\overset{\mbox{\tiny edit}}{\rightarrow}$};
        % \node[] at (1.15,3.0) {$\downarrow$};
        \node[] at (1.15,2.9) {\footnotesize Oedema};
        \node[] at (3.35,3.3) {\footnotesize Healthy $\overset{\mbox{\tiny edit}}{\rightarrow}$};
        % \node[] at (3.35,3.0) {$\downarrow$};
        \node[] at (3.35,2.9) {\footnotesize Pacemaker};
        \node[] at (5.55,3.3) {\footnotesize Healthy $\overset{\mbox{\tiny edit}}{\rightarrow}$};
        % \node[] at (5.55,3.0) {$\downarrow$};
        \node[] at (5.55,2.9) {\footnotesize Consolidation};

        % \node[] at (3.0,3.0) {\wip{(a) Evaluate with Hausdorff distance (AHD)}};
        % \node[] at (3.0,-1.5) {\wip{(b) Evaluate with Dice}};

        \matrix [draw,below left,fill=white] at (2.6,6.5) {
          \node[draw=myblue, fill=myblue,label=right:{\scriptsize Weak Predictor}] {}; \\
          \node[draw=myred, fill=myred,label=right:{\scriptsize Strong Predictor}] {}; \\
        };
        
        \end{tikzpicture}
        }
        \caption{Across edited datasets, a smaller increase in AHD is seen for the strong predictor model, demonstrating that it is less biased.}
    \end{subfigure}\hfill
    \begin{subfigure}{0.49\linewidth}
        \resizebox{\linewidth}{!}{
        \begin{tikzpicture}[
          every axis/.style={ % add these settings to all the axis environments in the tikzpicture
            width = 1.38\linewidth,
            height = 5cm,
            ybar stacked,
            ymajorgrids = true,
            major x tick style = transparent,
            ylabel = {},
            yticklabel style={/pgf/number format/fixed},
            xtick = \empty,
            axis line style={draw=none},
            enlarge x limits=0.25,
            bar width=14pt,
            symbolic x coords={
              Edema,
              Pacemaker,
              Consolidation,
            },
          },
        ]

        \draw[myred, line width=1pt] (0,1.41) -- (6.68,1.41);
        \draw[myblue, line width=1pt] (0,1.85) -- (6.68,1.85);

        % Set Dice 0 point. Here as MIMIC-Seg baseline
        \pgfmathsetmacro\diceaxis{1.0}

        % Dice MIMIC-Seg
        % bar shift -10pt here
        \pgfmathsetmacro\mimicdicereal{0.974}
        \pgfmathsetmacro\mimicdiceblank{\mimicdicereal-\diceaxis}
        \pgfmathsetmacro\mimicdiceedema{0.938-\mimicdiceblank-\diceaxis}
        \pgfmathsetmacro\mimicdicepacemaker{0.850-\mimicdiceblank-\diceaxis}
        \pgfmathsetmacro\mimicdiceconsolidation{0.859-\mimicdiceblank-\diceaxis}
        \begin{axis}[
            bar shift=-9pt,
            ymin=-0.15, ymax=0.0,
            ylabel = {$\Delta$ Dice score $\uparrow$},
            at={(0,-1cm)},
            % at={(0,-4cm)},
            ytick={0, -0.05, -0.1, -0.15},
            yticklabel={
                \pgfmathparse{\tick+\diceaxis}
                \pgfmathprintnumber{\pgfmathresult}
            }
        ]
            \addplot[draw=none] coordinates
            {
                (Edema,\mimicdiceblank) 
                (Pacemaker,\mimicdiceblank) 
                (Consolidation,\mimicdiceblank)
            };
            \addplot[black, fill=myblue] coordinates
            {
                (Edema,\mimicdiceedema) 
                (Pacemaker,\mimicdicepacemaker) 
                (Consolidation,\mimicdiceconsolidation)
            };
        \end{axis}

        % Dice CheXmask
        % zero bar shift here   
        \pgfmathsetmacro\chexmaskdicereal{0.955}
        \pgfmathsetmacro\chexmaskdiceblank{\chexmaskdicereal-\diceaxis}
        \pgfmathsetmacro\chexmaskdiceedema{0.919-\chexmaskdiceblank-\diceaxis}
        \pgfmathsetmacro\chexmaskdicepacemaker{0.873-\chexmaskdiceblank-\diceaxis}
        \pgfmathsetmacro\chexmaskdiceconsolidation{0.881-\chexmaskdiceblank-\diceaxis}
        \begin{axis}[
            bar shift=9pt,
            ymin=-0.15, ymax=0.0,
            at={(0,-1cm)},
            hide axis,
            yticklabel={
                \pgfmathparse{\tick+\diceaxis}
                \pgfmathprintnumber{\pgfmathresult}
            }
        ]
            \addplot[draw=none] coordinates
            {
                (Edema,\chexmaskdiceblank) 
                (Pacemaker,\chexmaskdiceblank) 
                (Consolidation,\chexmaskdiceblank)
            };
            \addplot+[black, fill=myred] coordinates
            {
                (Edema,\chexmaskdiceedema) 
                (Pacemaker,\chexmaskdicepacemaker) 
                (Consolidation,\chexmaskdiceconsolidation)
            };
        \end{axis}


        \node[] at (1.15,-1.3) {\footnotesize Healthy $\overset{\mbox{\tiny edit}}{\rightarrow}$};
        % \node[] at (1.15,3.0) {$\downarrow$};
        \node[] at (1.15,-1.7) {\footnotesize Oedema};
        \node[] at (3.35,-1.3) {\footnotesize Healthy $\overset{\mbox{\tiny edit}}{\rightarrow}$};
        % \node[] at (3.35,3.0) {$\downarrow$};
        \node[] at (3.35,-1.7) {\footnotesize Pacemaker};
        \node[] at (5.55,-1.3) {\footnotesize Healthy $\overset{\mbox{\tiny edit}}{\rightarrow}$};
        % \node[] at (5.55,3.0) {$\downarrow$};
        \node[] at (5.55,-1.7) {\footnotesize Consolidation};

        % \node[] at (3.0,3.0) {\wip{(a) Evaluate with Hausdorff distance (AHD)}};
        % \node[] at (3.0,-1.5) {\wip{(b) Evaluate with Dice}};

        \matrix [draw,below left,fill=white] at (2.6,0.3) {
          \node[draw=myblue, fill=myblue,label=right:{\scriptsize Weak Predictor}] {}; \\
          \node[draw=myred, fill=myred,label=right:{\scriptsize Strong Predictor}] {}; \\
        };
        
        \end{tikzpicture}
        }
        \caption{Across edited datasets, a smaller decrease in Dice score is seen for the strong predictor model, demonstrating that it is less biased.}
    \end{subfigure}
    \caption{\textbf{Quantifying robustness of lung segmentation models to population shift}. We evaluate a `weak predictor' trained on MIMIC-Seg (a small set of predominantly healthy patients), shown in \textcolor{myblue}{blue}, a `strong predictor' trained on CheXmask (a large mixed set of patients with more abnormalities), shown in \textcolor{myred}{red}; reporting the change in Dice score and \ac{AHD} after editing in oedema, pacemakers, and consolidation, with respect to the models evaluated on the ground truth test set (baseline values shown as horizontal lines).}
    \label{fig:segmentation-bar-chart}
    \vspace{-1em}
\end{figure}


